Predicate Invention for Bilevel Planning

Efficient planning in continuous state and action spaces is fundamentally hard, even when the transition model is deterministic and known. One way to alleviate this challenge is to perform bilevel planning with abstractions, where a high-level search for abstract plans is used to guide planning in the original transition space. Previous work has shown that when state abstractions in the form of symbolic predicates are hand-designed, operators and samplers for bilevel planning can be learned from demonstrations. In this work, we propose an algorithm for learning predicates from demonstrations, eliminating the need for manually specified state abstractions. Our key idea is to learn predicates by optimizing a surrogate objective that is tractable but faithful to our real efficient-planning objective. We use this surrogate objective in a hill-climbing search over predicate sets drawn from a grammar. Experimentally, we show across four robotic planning environments that our learned abstractions are able to quickly solve held-out tasks, outperforming six baselines. Code: https://tinyurl.com/predicators-release

==> results_table.tex <==
\begin{table*}
	\centering
	\scriptsize
\begin{tabular}{| l | p{0.49cm} | p{0.49cm} || p{0.49cm} | p{0.49cm} || p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} || p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | }
	\hline
	\multicolumn{1}{|c|}{} &\multicolumn{2}{c||}{\bf{Ours}} &
	\multicolumn{2}{c||}{\bf{Manual}} &
	\multicolumn{2}{c|}{\bf{Down Learn}} &
	\multicolumn{2}{c|}{\bf{Down Eval}} &
	\multicolumn{2}{c||}{\bf{No Invent}} &
	\multicolumn{2}{c|}{\bf{Bisimulation}} &
	\multicolumn{2}{c|}{\bf{Branching}} &
	\multicolumn{2}{c|}{\bf{Boltzmann}} &
	\multicolumn{2}{c|}{\bf{Random}} \\
	\hline
	\bf{Environment} &
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}\\
	\hline
	PickPlace1D & 99.6 & 0.006 & 99.8 & 0.113 & 99.8 & 0.006 & 99.6 & 0.006 & 23.4 & 0.003 & 99.8 & 0.006 & 23.4 & 0.003 & 99.8 & 0.005 & 16.8 & 0.007 \\
	Blocks & 100.0 & 0.375 & 100.0 & 0.295 & 84.6 & 0.443 & 100.0 & 0.370 & 1.6 & 4.221 & 14.6 & 0.948 & 100.0 & 0.366 & 79.6 & 0.829 & 0.2 & 0.020 \\
	Painting & 96.4 & 0.201 & 99.8 & 0.433 & 99.8 & 0.196 & 95.6 & 0.207 & 0.0 & \;\;\;-- & 0.0 & \;\;\;-- & 8.6 & 4.778 & 99.2 & 0.769 & 0.0 & \;\;\;-- \\
	Tools & 96.6 & 0.489 & 99.4 & 0.638 & 97.4 & 0.477 & 48.8 & 0.075 & 0.0 & \;\;\;-- & 25.8 & 1.036 & 73.6 & 0.097 & 62.6 & 0.303 & 0.0 & \;\;\;-- \\\hline
	\end{tabular}
	\caption{\small{\textbf{Main results.} Percentage of 50 evaluation tasks solved under a 10-second timeout (Succ), and average planning time in seconds over successful tasks (Time). All numbers are averages over 10 seeds, which vary the training and evaluation tasks, random initializations during learning, and tiebreaking during planning. Standard deviations and learning times are  in \appref{app:results}. Our learned abstractions (Ours) perform extremely well compared to all baselines (rightmost four columns), and can even lead to more efficient planning than is obtained using manually designed state abstractions (Manual).}}
	\label{tab:mainresults}
	\vspace{-2.75em}
\end{table*}

==> stds_main_results_table.tex <==
\begin{table*}
	\centering
	\scriptsize
\begin{tabular}{| l | p{0.49cm} | p{0.49cm} || p{0.49cm} | p{0.49cm} || p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} || p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | p{0.49cm} | }
	\hline
	\multicolumn{1}{|c|}{} &\multicolumn{2}{c||}{\bf{Ours}} &
	\multicolumn{2}{c||}{\bf{Manual}} &
	\multicolumn{2}{c|}{\bf{Down Learn}} &
	\multicolumn{2}{c|}{\bf{Down Eval}} &
	\multicolumn{2}{c||}{\bf{No Invent}} &
	\multicolumn{2}{c|}{\bf{Bisimulation}} &
	\multicolumn{2}{c|}{\bf{Branching}} &
	\multicolumn{2}{c|}{\bf{Boltzmann}} &
	\multicolumn{2}{c|}{\bf{Random}} \\
	\hline
	\bf{Environment} &
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}&
	{\scriptsize Succ} & {\scriptsize Time}\\
	\hline
	PickPlace1D & 1.2 & 0.001 & 0.6 & 0.041 & 0.6 & 0.001 & 1.2 & 0.002 & 7.4 & 0.002 & 0.6 & 0.000 & 7.4 & 0.002 & 0.6 & 0.000 & 3.7 & 0.002 \\
	Blocks & 0.0 & 0.102 & 0.0 & 0.075 & 24.9 & 0.172 & 0.0 & 0.105 & 1.5 & 3.014 & 3.7 & 0.907 & 0.0 & 0.101 & 13.4 & 0.363 & 0.6 & 0.000 \\
	Painting & 10.2 & 0.026 & 0.6 & 0.065 & 0.6 & 0.016 & 9.2 & 0.037 & 0.0 & \;\;\;-- & 0.0 & \;\;\;-- & 8.1 & 1.953 & 1.0 & 0.570 & 0.0 & \;\;\;-- \\
	Tools & 4.8 & 0.177 & 0.9 & 0.126 & 3.5 & 0.212 & 10.7 & 0.021 & 0.0 & \;\;\;-- & 2.3 & 0.362 & 10.7 & 0.043 & 4.5 & 0.064 & 0.0 & \;\;\;-- \\\hline
	\end{tabular}
	\caption{Standard deviations for the corresponding entries in \tabref{tab:ablations}, which were all means over 10 random seeds.}
	\label{tab:stdmainresults}
\end{table*}
